High Energy Physics Opportunities Using Reactor Antineutrinos

Nuclear reactors are uniquely powerful, abundant, and flavor-pure sources of antineutrinos that continue to play a vital role in the US neutrino physics program. The US reactor antineutrino physics community is a diverse interest group encompassing many detection technologies and many particle physics topics, including Standard Model and short-baseline oscillations, BSM physics searches, and reactor flux and spectrum modeling. The community's aims offer strong complimentary with numerous aspects of the wider US neutrino program and have direct relevance to most of the topical sub-groups composing the Snowmass 2021 Neutrino Frontier. Reactor neutrino experiments also have a direct societal impact and have become a strong workforce and technology development pipeline for DOE National Laboratories and universities. This white paper, prepared as a submission to the Snowmass 2021 community organizing exercise, will survey the state of the reactor antineutrino physics field and summarize the ways in which current and future reactor antineutrino experiments can play a critical role in advancing the field of particle physics in the next decade.

==> AuthorListJun2021.tex <==
% !TEX root = main.tex

\newcommand{\NCSDLLNL}{\affiliation{Lawrence Livermore National Laboratory, Livermore, CA, USA}}
\newcommand{\IIT}{\affiliation{Department of Physics, Illinois Institute of Technology, Chicago, IL, USA}}
\newcommand{\USNA}{\affiliation{Department of Physics, United States Naval Academy, Annapolis, MD, USA}}
\newcommand{\UCB}{\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}}
\newcommand{\INT}{\affiliation{Institute for Nuclear Theory, University of Washington, Seattle, WA 98195, USA}}
\newcommand{\UCI}{\affiliation{Department of Physics and Astronomy, University of California, Irvine, California 92697}}
\newcommand{\ORNL}{\affiliation{Oak Ridge National Laboratory, Oak Ridge, TN, USA}}
\newcommand{\FNAL}{\affiliation{\normalsize Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA.}}
\newcommand{\BNL}{\affiliation{\normalsize Physics Department, Brookhaven National Laboratory, Upton, NY 11973, USA}}
\newcommand{\LBNL}{\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}}
\newcommand{\Yale}{\affiliation{Wright Laboratory and Department of Physics, Yale University, New Haven, CT, 06511 USA}}
\newcommand{\VT}{\affiliation{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, USA}}

\author{O.\,A.\,Akindele}\NCSDLLNL
\author{J.\,M.\,Berryman}\UCB\\\INT
\author{N.\,S.\,Bowden}\NCSDLLNL
\author{R.\,Carr}\USNA
\author{A.\,J.\,Conant}\ORNL
\author{G.\,Fernandez-Moroni}\FNAL
\author{P.\,Huber}\VT
\author{T.\,J.\,Langford}\Yale
\author{B.\,R.\,Littlejohn}\IIT
\author{J.\,P.\,Ochoa-Ricoux}\UCI
\author{C.\,Roca}\NCSDLLNL
\author{S.\,Schoppmann}\UCB\\\LBNL
\author{J.\,Xu}\NCSDLLNL
\author{C.\,Zhang}\BNL
\author{X.\,Zhang}\NCSDLLNL


%\author{B~R~Littlejohn$^{ 6}$,R~Carr$^{}$, J~M~Berryman$^{a,b}$}

%\address{$^{6}$Department of Physics, Illinois Institute of Technology, Chicago, IL, US} \vspace{-0.4\baselineskip}
%\address{$^{}$Department of Physics, United States Naval Academy, Annapolis, MD, US}
%\address{$^{a}$Department of Physics, University of California, Berkeley, CA 94720, USA}
%\address{$^{b}$Institute for Nuclear Theory, University of Washington, Seattle, WA 98195, USA}

==> FullAuthorList.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
%Chandler
%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\VirginiaTech}{\affiliation{Center for Neutrino Physics, Virginia~Tech, Blacksburg, Virginia  24061}}
\newcommand{\Duke}{\affiliation{Department of Physics, Duke University, Durham, NC 27708}}
\newcommand{\TUNL}{\affiliation{Triangle Universities Nuclear Laboratory, Durham, NC 27708}}
\author{C.~Awe}\Duke\TUNL
\author{P.S.~Barbeau}\Duke\TUNL
\author{A.~Haghighat}\VirginiaTech
\author{P.~Huber}\VirginiaTech
\author{S.~C.~Li}\VirginiaTech
\author{J.M.~Link}\VirginiaTech
\author{V.~Mascolino}\VirginiaTech
\author{T.~Subedi}\VirginiaTech
\author{K.~Walkup}\VirginiaTech
\collaboration{The CHANDLER Collaboration}
\noaffiliation

%%%%%%%%%%%%%%%%%%%%%%%%
%CONNIE
%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\UNAM}{\affiliation{Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}}
\newcommand{\CABIB}{\affiliation{Centro At\'omico Bariloche and Instituto Balseiro, Comisi\'on Nacional de Energ\'ia At\'omica (CNEA), Consejo Nacional de Investigaciones Cient\'ificas y T\'ecnicas (CONICET), Universidad Nacional de Cuyo (UNCUYO), San Carlos de Bariloche, Argentina.}}
\newcommand{\UFRJ}{\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'isica, Rio de Janeiro, RJ, Brazil}}
\newcommand{\FNAL}{\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, United States}}
\newcommand{\FIUNA}{\affiliation{Facultad de Ingenier\'ia - Universidad Nacional de Asunci\'on, Asunci\'on, Paraguay}}
\newcommand{\CBPFRJ}{\affiliation{Centro Brasileiro de Pesquisas F\'isicas, Rio de Janeiro, RJ, Brazil}}
\newcommand{\CFETCSF}{\affiliation{Centro Federal de Educa\c c\~ao Tecnol\'ogica Celso Suckow da Fonseca, Angra dos Reis, RJ, Brazil}}
\newcommand{\IIIE}{\affiliation{Instituto de Investigaciones en Ingenier\'ia El\'ectrica, Departamento de Ingenier\'ia El\'ectrica y Computadoras, Universidad Nacional del Sur (UNS) - CONICET, Bah\'ia Blanca, Argentina}}
\newcommand{\UNSAM}{\affiliation{Universidad Nacional de San Mart\'in (UNSAM), Comisi\'on Nacional de Energ\'ia At\'omica (CNEA),  Consejo Nacional de Investigaciones Cient\'ificas y T\'ecnicas (CONICET), Argentina}}
\newcommand{\UZPI}{\affiliation{Universit\"at Z\"urich Physik Institut, Zurich, Switzerland}}

\author{A.~Aguilar-Arevalo}\UNAM
\author{X.~Bertou}\CABIB
\author{C.~Bonifazi}\UFRJ
\author{G.~Cancelo}\FNAL
\author{B.~A.~Cervantes-Vergara}\UNAM
\author{C.~Chavez}\FIUNA
\author{J.~C.~D'Olivo}\UNAM
\author{J.~M..~De Egea}\FIUNA
\author{J.~C.~dos Anjos}\CBPFRJ
\author{J.~Estrada}\FNAL
\author{A.~R.~F.~Neto}\CFETCSF
\author{G.~Fernandez-Moroni}\FNAL\IIIE
\author{A.~Foguel}\UFRJ
\author{R.~Ford}\FNAL
\author{J.~Gasanego}\UNSAM
\author{V.~Gollo}\UFRJ
\author{F.~Izraelevitch}\UNSAM
\author{B.~Kilminster}\UZPI
\author{H.~P.~Lima Jr}\CBPFRJ
\author{M.~Makler}\CBPFRJ
\author{L.~H.~Mendes}\UFRJ
\author{J.~Molina}\FIUNA
\author{P.~Mota}\CBPFRJ
\author{I.~Nasteva}\UFRJ
\author{E.~Paolini}\IIIE
\author{C.~Romero}\FIUNA
\author{Y.~Sarkis}\UNAM
\author{M.~S.~Haro}\CABIB
\author{A.~Soto}\IIIE
\author{D.~Stalder}\FIUNA
\author{J.~Tiffenberg}\FNAL
\author{C.~Torres}\FIUNA
\collaboration{The CONNIE Collaboration}
\noaffiliation

%%%%%%%%%%%%%%%%%%%%%%%%
%CONUS
%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\MPIK}{\affiliation{Max-Planck-Institut f\"ur Kernphysik, Saupfercheckweg 1, 69117 Heidelberg, Germany}}

\author{M.~Lindner}\MPIK
\collaboration{on behalf of The CONUS Collaboration}
\noaffiliation

%%%%%%%%%%%%%%%%%%%%%%%%
%Daya Bay
%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ECUST}{\affiliation{Institute of Modern Physics, East China University of Science and Technology, Shanghai}}
\newcommand{\IHEP}{\affiliation{Institute~of~High~Energy~Physics, Beijing}}
\newcommand{\Wisconsin}{\affiliation{University~of~Wisconsin, Madison, Wisconsin 53706}}
\newcommand{\Yale}{\affiliation{Wright~Laboratory and Department~of~Physics, Yale~University, New~Haven, Connecticut 06520}} %%%% 20170227 add Wright Lab
\newcommand{\BNL}{\affiliation{Brookhaven~National~Laboratory, Upton, New York 11973}}
\newcommand{\NTU}{\affiliation{Department of Physics, National~Taiwan~University, Taipei}}
\newcommand{\NUU}{\affiliation{National~United~University, Miao-Li}}
\newcommand{\Dubna}{\affiliation{Joint~Institute~for~Nuclear~Research, Dubna, Moscow~Region}}
\newcommand{\CalTech}{\affiliation{California~Institute~of~Technology, Pasadena, California 91125}}
\newcommand{\CUHK}{\affiliation{Chinese~University~of~Hong~Kong, Hong~Kong}}
\newcommand{\NCTU}{\affiliation{Institute~of~Physics, National~Chiao-Tung~University, Hsinchu}}
\newcommand{\NJU}{\affiliation{Nanjing~University, Nanjing}}
\newcommand{\JUNOM}{\affiliation{Department~of~Engineering~Physics, JUNOM~University, Beijing}}
\newcommand{\SZU}{\affiliation{Shenzhen~University, Shenzhen}}
\newcommand{\NCEPU}{\affiliation{North~China~Electric~Power~University, Beijing}}
\newcommand{\Siena}{\affiliation{Siena~College, Loudonville, New York  12211}}
\newcommand{\IIT}{\affiliation{Department of Physics, Illinois~Institute~of~Technology, Chicago, Illinois  60616}}
\newcommand{\LBNL}{\affiliation{Lawrence~Berkeley~National~Laboratory, Berkeley, California 94720}}
\newcommand{\UIUC}{\affiliation{Department of Physics, University~of~Illinois~at~Urbana-Champaign, Urbana, Illinois 61801}}
\newcommand{\SJTU}{\affiliation{Department of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai Laboratory for Particle Physics and Cosmology, Shanghai}}
\newcommand{\BNU}{\affiliation{Beijing~Normal~University, Beijing}}
\newcommand{\WM}{\affiliation{College~of~William~and~Mary, Williamsburg, Virginia  23187}}
\newcommand{\Princeton}{\affiliation{Joseph Henry Laboratories, Princeton~University, Princeton, New~Jersey 08544}}
\newcommand{\CIAE}{\affiliation{China~Institute~of~Atomic~Energy, Beijing}}
\newcommand{\SDU}{\affiliation{Shandong~University, Jinan}}
\newcommand{\NanKai}{\affiliation{School of Physics, Nankai~University, Tianjin}}
\newcommand{\UC}{\affiliation{Department of Physics, University~of~Cincinnati, Cincinnati, Ohio 45221}}
\newcommand{\DGUT}{\affiliation{Dongguan~University~of~Technology, Dongguan}}
\newcommand{\XJTU}{\affiliation{Department of Nuclear Science and Technology, School of Energy and Power Engineering, Xi'an Jiaotong University, Xi'an}}%%updated 20161215 {Xi'an Jiaotong University, Xi'an}}
\newcommand{\UCB}{\affiliation{Department of Physics, University~of~California, Berkeley, California  94720}}
\newcommand{\HKU}{\affiliation{Department of Physics, The~University~of~Hong~Kong, Pokfulam, Hong~Kong}}
\newcommand{\UIAH}{\affiliation{Department of Physics, University~of~Houston, Houston, Texas  77204}}
\newcommand{\Charles}{\affiliation{Charles~University, Faculty~of~Mathematics~and~Physics, Prague}} %updated20140819
\newcommand{\USTC}{\affiliation{University~of~Science~and~Technology~of~China, Hefei}}
\newcommand{\TempleUniversity}{\affiliation{Department~of~Physics, College~of~Science~and~Technology, Temple~University, Philadelphia, Pennsylvania  19122}}
\newcommand{\CGNPG}{\affiliation{China General Nuclear Power Group, Shenzhen}}% update 20170729 add city. updated 20140724 China~Guangdong~Nuclear~Power~Group, Shenzhen}}
\newcommand{\NUDT}{\affiliation{College of Electronic Science and Engineering, National University of Defense Technology, Changsha}} % added 20140111
\newcommand{\IowaState}{\affiliation{Iowa~State~University, Ames, Iowa  50011}}
\newcommand{\ZSU}{\affiliation{Sun Yat-Sen (Zhongshan) University, Guangzhou}}
\newcommand{\CQU}{\affiliation{Chongqing University, Chongqing}} % add 20150417
%\newcommand{\BCC}{\altaffiliation[Now at ]{Department of Chemistry and Chemical Technology, Bronx Community College, Bronx, New York  10453}} % add 20160311 for Sunej's 'now at'

\newcommand{\UCI}{\affiliation{Department of Physics and Astronomy, University of California, Irvine, California 92697}} %20190209 for Pedro's new digs
\author{F.~P.~An}\ECUST
\author{A.~B.~Balantekin}\Wisconsin
\author{H.~R.~Band}\Yale
\author{M.~Bishai}\BNL
\author{S.~Blyth}\NTU
\author{G.~F.~Cao}\IHEP
\author{J.~Cao}\IHEP
\author{J.~F.~Chang}\IHEP
\author{Y.~Chang}\NUU
\author{H.~S.~Chen}\IHEP
\author{S.~M.~Chen}\JUNOM
\author{Y.~Chen}\SZU\ZSU
\author{Y.~X.~Chen}\NCEPU
\author{J.~Cheng}\IHEP
\author{Z.~K.~Cheng}\ZSU
\author{J.~J.~Cherwinka}\Wisconsin
\author{M.~C.~Chu}\CUHK
\author{J.~P.~Cummings}\Siena
\author{O.~Dalager}\UCI
\author{F.~S.~Deng}\USTC
\author{Y.~Y.~Ding}\IHEP
\author{M.~V.~Diwan}\BNL
\author{T.~Dohnal}\Charles
\author{J.~Dove}\UIUC
\author{M.~Dvo\v{r}\'{a}k}\Charles
\author{D.~A.~Dwyer}\LBNL
\author{J.~P.~Gallo}\IIT
\author{M.~Gonchar}\Dubna
\author{G.~H.~Gong}\JUNOM
\author{H.~Gong}\JUNOM
\author{W.~Q.~Gu}\BNL
\author{J.~Y.~Guo}\ZSU
\author{L.~Guo}\JUNOM
\author{X.~H.~Guo}\BNU
\author{Y.~H.~Guo}\XJTU
\author{Z.~Guo}\JUNOM
\author{R.~W.~Hackenburg}\BNL
\author{S.~Hans}\BNL
\author{M.~He}\IHEP
\author{K.~M.~Heeger}\Yale
\author{Y.~K.~Heng}\IHEP
\author{A.~Higuera}\UIAH
\author{Y.~K.~Hor}\ZSU
\author{Y.~B.~Hsiung}\NTU
\author{B.~Z.~Hu}\NTU
\author{J.~R.~Hu}\IHEP
\author{T.~Hu}\IHEP
\author{Z.~J.~Hu}\ZSU
\author{H.~X.~Huang}\CIAE
\author{X.~T.~Huang}\SDU
\author{P.~Huber}\VirginiaTech
\author{D.~E.~Jaffe}\BNL
\author{K.~L.~Jen}\NCTU
\author{X.~L.~Ji}\IHEP
\author{X.~P.~Ji}\BNL
\author{R.~A.~Johnson}\UC
\author{D.~Jones}\TempleUniversity
\author{L.~Kang}\DGUT
\author{S.~H.~Kettell}\BNL
\author{S.~Kohn}\UCB
\author{M.~Kramer}\LBNL\UCB
\author{T.~J.~Langford}\Yale
\author{J.~Lee}\LBNL
\author{J.~H.~C.~Lee}\HKU
\author{R.~T.~Lei}\DGUT
\author{R.~Leitner}\Charles
\author{J.~K.~C.~Leung}\HKU
\author{F.~Li}\IHEP
\author{H.~L.~Li}\IHEP
\author{J.~J.~Li}\JUNOM
\author{Q.~J.~Li}\IHEP
\author{S.~Li}\DGUT
\author{S.~C.~Li}\VirginiaTech
\author{W.~D.~Li}\IHEP
\author{X.~N.~Li}\IHEP
\author{X.~Q.~Li}\NanKai
\author{Y.~F.~Li}\IHEP
\author{Z.~B.~Li}\ZSU
\author{H.~Liang}\USTC
\author{C.~J.~Lin}\LBNL
\author{G.~L.~Lin}\NCTU
\author{S.~Lin}\DGUT
\author{J.~J.~Ling}\ZSU
\author{J.~M.~Link}\VirginiaTech
\author{L.~Littenberg}\BNL
\author{B.~R.~Littlejohn}\IIT
\author{J.~C.~Liu}\IHEP
\author{J.~L.~Liu}\SJTU
\author{C.~Lu}\Princeton
\author{H.~Q.~Lu}\IHEP
\author{J.~S.~Lu}\IHEP
\author{K.~B.~Luk}\UCB\LBNL
\author{X.~B.~Ma}\NCEPU
\author{X.~Y.~Ma}\IHEP
\author{Y.~Q.~Ma}\IHEP
\author{R.~C.~Mandujano}\UCI
\author{C.~Marshall}\LBNL
\author{D.~A.~Martinez Caicedo}\IIT
\author{K.~T.~McDonald}\Princeton
\author{R.~D.~McKeown}\CalTech\WM
\author{Y.~Meng}\SJTU
\author{J.~Napolitano}\TempleUniversity
\author{D.~Naumov}\Dubna
\author{E.~Naumova}\Dubna
\author{J.~P.~Ochoa-Ricoux}\UCI
\author{A.~Olshevskiy}\Dubna
\author{H.-R.~Pan}\NTU
\author{J.~Park}\VirginiaTech
\author{S.~Patton}\LBNL
\author{J.~C.~Peng}\UIUC
\author{C.~S.~J.~Pun}\HKU
\author{F.~Z.~Qi}\IHEP
\author{M.~Qi}\NJU
\author{X.~Qian}\BNL
\author{N.~Raper}\ZSU
\author{J.~Ren}\CIAE
\author{C.~Morales~Reveco}\UCI
\author{R.~Rosero}\BNL
\author{B.~Roskovec}\UCI
\author{X.~C.~Ruan}\CIAE
\author{H.~Steiner}\UCB\LBNL
\author{J.~L.~Sun}\CGNPG
\author{T.~Tmej}\Charles
\author{K.~Treskov}\Dubna
\author{W.-H.~Tse}\CUHK
\author{C.~E.~Tull}\LBNL
\author{B.~Viren}\BNL
\author{V.~Vorobel}\Charles
\author{C.~H.~Wang}\NUU
\author{J.~Wang}\ZSU
\author{M.~Wang}\SDU
\author{N.~Y.~Wang}\BNU
\author{R.~G.~Wang}\IHEP
\author{W.~Wang}\ZSU\WM
\author{W.~Wang}\NJU
\author{X.~Wang}\NUDT
\author{Y.~Wang}\NJU
\author{Y.~F.~Wang}\IHEP
\author{Z.~Wang}\IHEP
\author{Z.~Wang}\JUNOM
\author{Z.~M.~Wang}\IHEP
\author{H.~Y.~Wei}\BNL
\author{L.~H.~Wei}\IHEP
\author{L.~J.~Wen}\IHEP
\author{K.~Whisnant}\IowaState
\author{C.~G.~White}\IIT
\author{H.~L.~H.~Wong}\UCB\LBNL
\author{E.~Worcester}\BNL
\author{D.~R.~Wu}\IHEP
\author{F.~L.~Wu}\NJU
\author{Q.~Wu}\SDU
\author{W.~J.~Wu}\IHEP
\author{D.~M.~Xia}\CQU
\author{Z.~Q.~Xie}\IHEP
\author{Z.~Z.~Xing}\IHEP
\author{J.~L.~Xu}\IHEP
\author{T.~Xu}\JUNOM
\author{T.~Xue}\JUNOM
\author{C.~G.~Yang}\IHEP
\author{L.~Yang}\DGUT
\author{Y.~Z.~Yang}\JUNOM
\author{H.~F.~Yao}\IHEP
\author{M.~Ye}\IHEP
\author{M.~Yeh}\BNL
\author{B.~L.~Young}\IowaState
\author{H.~Z.~Yu}\ZSU
\author{Z.~Y.~Yu}\IHEP
\author{B.~B.~Yue}\ZSU
\author{S.~Zeng}\IHEP
\author{Y.~Zeng}\ZSU
\author{L.~Zhan}\IHEP
\author{C.~Zhang}\BNL
\author{F.~Y.~Zhang}\SJTU
\author{H.~H.~Zhang}\ZSU
\author{J.~W.~Zhang}\IHEP
\author{Q.~M.~Zhang}\XJTU
\author{X.~T.~Zhang}\IHEP
\author{Y.~M.~Zhang}\ZSU
\author{Y.~X.~Zhang}\CGNPG
\author{Y.~Y.~Zhang}\SJTU
\author{Z.~J.~Zhang}\DGUT
\author{Z.~P.~Zhang}\USTC
\author{Z.~Y.~Zhang}\IHEP
\author{J.~Zhao}\IHEP
\author{L.~Zhou}\IHEP
\author{H.~L.~Zhuang}\IHEP
\author{J.~H.~Zou}\IHEP
\collaboration{The Daya Bay Collaboration}
\noaffiliation

%%%%%%%%%%%%%%%%%%%%%%%%
%JUNO
%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\JUNOA}{\affiliation{Yerevan Physics Institute, Yerevan, Armenia}}
\newcommand{\JUNOB}{\affiliation{Universit\'{e} Libre de Bruxelles, Brussels, Belgium}}
\newcommand{\JUNOC}{\affiliation{Universidade Estadual de Londrina, Londrina, Brazil}}
\newcommand{\JUNOD}{\affiliation{Pontificia Universidade Catolica do Rio de Janeiro, Rio, Brazil}}
\newcommand{\JUNOE}{\affiliation{Pontificia Universidad Cat\'{o}lica de Chile, Santiago, Chile}}
\newcommand{\JUNOF}{\affiliation{Universidad Tecnica Federico Santa Maria, Valparaiso, Chile}}
\newcommand{\JUNOG}{\affiliation{Beijing Institute of Spacecraft Environment Engineering, Beijing, China}}
\newcommand{\JUNOH}{\affiliation{Beijing Normal University, Beijing, China}}
\newcommand{\JUNOI}{\affiliation{China Institute of Atomic Energy, Beijing, China}}
\newcommand{\JUNOJ}{\affiliation{Institute of High Energy Physics, Beijing, China}}
\newcommand{\JUNOK}{\affiliation{North China Electric Power University, Beijing, China}}
\newcommand{\JUNOL}{\affiliation{School of Physics, Peking University, Beijing, China}}
\newcommand{\TSINGHUA}{\affiliation{Tsinghua University, Beijing, China}}
\newcommand{\JUNON}{\affiliation{University of Chinese Academy of Sciences, Beijing, China}}
\newcommand{\JUNOO}{\affiliation{Jilin University, Changchun, China}}
\newcommand{\JUNOP}{\affiliation{College of Electronic Science and Engineering, National University of Defense Technology, Changsha, China}}
\newcommand{\JUNOQ}{\affiliation{Chongqing University, Chongqing, China}}
\newcommand{\JUNOR}{\affiliation{Dongguan University of Technology, Dongguan, China}}
\newcommand{\JUNOS}{\affiliation{Jinan University, Guangzhou, China}}
\newcommand{\JUNOT}{\affiliation{Sun Yat-Sen University, Guangzhou, China}}
\newcommand{\JUNOU}{\affiliation{Harbin Institute of Technology, Harbin, China}}
\newcommand{\JUNOV}{\affiliation{University of Science and Technology of China, Hefei, China}}
\newcommand{\JUNOW}{\affiliation{The Radiochemistry and Nuclear Chemistry Group in University of South China, Hengyang, China}}
\newcommand{\JUNOX}{\affiliation{Wuyi University, Jiangmen, China}}
\newcommand{\JUNOY}{\affiliation{Shandong University, Jinan, China}}
\newcommand{\JUNOZ}{\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, China}}
\newcommand{\JUNOAA}{\affiliation{Nanjing University, Nanjing, China}}
\newcommand{\JUNOAB}{\affiliation{Guangxi University, Nanning, China}}
\newcommand{\JUNOAC}{\affiliation{East China University of Science and Technology, Shanghai, China}}
\newcommand{\JUNOAD}{\affiliation{School of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai, China}}
\newcommand{\JUNOAE}{\affiliation{Tsung-Dao Lee Institute, Shanghai Jiao Tong University, Shanghai, China}}
\newcommand{\JUNOAF}{\affiliation{Institute of Hydrogeology and Environmental Geology, Chinese Academy of Geological Sciences, Shijiazhuang, China}}
\newcommand{\JUNOAG}{\affiliation{Nankai University, Tianjin, China}}
\newcommand{\JUNOAH}{\affiliation{Wuhan University, Wuhan, China}}
\newcommand{\JUNOAI}{\affiliation{Xi'an Jiaotong University, Xi'an, China}}
\newcommand{\JUNOAJ}{\affiliation{Xiamen University, Xiamen, China}}
\newcommand{\JUNOAK}{\affiliation{School of Physics and Microelectronics, Zhengzhou University, Zhengzhou, China}}
\newcommand{\JUNOAL}{\affiliation{Institute of Physics National Chiao-Tung University, Hsinchu}}
\newcommand{\JUNOAM}{\affiliation{National United University, Miao-Li}}
\newcommand{\JUNOAN}{\affiliation{Department of Physics, National Taiwan University, Taipei}}
\newcommand{\JUNOAO}{\affiliation{Charles University, Faculty of Mathematics and Physics, Prague, Czech Republic}}
\newcommand{\JUNOAP}{\affiliation{University of Jyvaskyla, Department of Physics, Jyvaskyla, Finland}}
\newcommand{\JUNOAQ}{\affiliation{IJCLab, Universit\'{e} Paris-Saclay, CNRS/IN2P3, 91405 Orsay, France}}
\newcommand{\JUNOAR}{\affiliation{Universit\'{e} de Bordeaux, CNRS, CENBG-IN2P3, F-33170 Gradignan, France}}
\newcommand{\JUNOAS}{\affiliation{IPHC, Universit\'{e} de Strasbourg, CNRS/IN2P3, F-67037 Strasbourg, France}}
\newcommand{\JUNOAT}{\affiliation{Centre de Physique des Particules de Marseille, Marseille, France}}
\newcommand{\JUNOAU}{\affiliation{SUBATECH, Universit\'{e} de Nantes,  IMT Atlantique, CNRS-IN2P3, Nantes, France}}
\newcommand{\JUNOAV}{\affiliation{III. Physikalisches Institut B, RWTH Aachen University, Aachen, Germany}}
\newcommand{\JUNOAW}{\affiliation{Institute of Experimental Physics, University of Hamburg, Hamburg, Germany}}
\newcommand{\JUNOAX}{\affiliation{Forschungszentrum J\"{u}lich GmbH, Nuclear Physics Institute IKP-2, J\"{u}lich, Germany}}
\newcommand{\JUNOAY}{\affiliation{Forschungszentrum J\"{u}lich GmbH, Central Institute of Engineering, Electronics and Analytics - Electronic Systems(ZEA-2), J\"{u}lich, Germany}}
\newcommand{\JUNOAZ}{\affiliation{Institute of Physics, Johannes-Gutenberg Universit\"{a}t Mainz, Mainz, Germany}}
\newcommand{\JUNOBA}{\affiliation{Technische Universit\"{a}t M\"{u}nchen, M\"{u}nchen, Germany}}
\newcommand{\JUNOBB}{\affiliation{Eberhard Karls Universit\"{a}t T\"{u}bingen, Physikalisches Institut, T\"{u}bingen, Germany}}
\newcommand{\JUNOBC}{\affiliation{INFN Catania and Dipartimento di Fisica e Astronomia dell Universit\`{a} di Catania, Catania, Italy}}
\newcommand{\JUNOBD}{\affiliation{INFN Catania and Centro Siciliano di Fisica Nucleare e Struttura della Materia, Catania, Italy}}
\newcommand{\JUNOBE}{\affiliation{Department of Physics and Earth Science, University of Ferrara and INFN Sezione di Ferrara, Ferrara, Italy}}
\newcommand{\JUNOBF}{\affiliation{INFN Sezione di Milano and Dipartimento di Fisica dell Universit\`{a} di Milano, Milano, Italy}}
\newcommand{\JUNOBG}{\affiliation{INFN Milano Bicocca and University of Milano Bicocca, Milano, Italy}}
\newcommand{\JUNOBH}{\affiliation{INFN Milano Bicocca and Politecnico of Milano, Milano, Italy}}
\newcommand{\JUNOBI}{\affiliation{INFN Sezione di Padova, Padova, Italy}}
\newcommand{\JUNOBJ}{\affiliation{Dipartimento di Fisica e Astronomia dell'Universita' di Padova and INFN Sezione di Padova, Padova, Italy}}
\newcommand{\JUNOBK}{\affiliation{INFN Sezione di Perugia and Dipartimento di Chimica, Biologia e Biotecnologie dell'Universit\`{a} di Perugia, Perugia, Italy}}
\newcommand{\JUNOBL}{\affiliation{Laboratori Nazionali di Frascati dell'INFN, Roma, Italy}}
\newcommand{\JUNOBM}{\affiliation{University of Roma Tre and INFN Sezione Roma Tre, Roma, Italy}}
\newcommand{\JUNOBN}{\affiliation{Institute of Electronics and Computer Science, Riga, Latvia}}
\newcommand{\JUNOBO}{\affiliation{Pakistan Institute of Nuclear Science and Technology, Islamabad, Pakistan}}
\newcommand{\JUNOBP}{\affiliation{Joint Institute for Nuclear Research, Dubna, Russia}}
\newcommand{\JUNOBQ}{\affiliation{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}}
\newcommand{\JUNOBR}{\affiliation{Lomonosov Moscow State University, Moscow, Russia}}
\newcommand{\JUNOBS}{\affiliation{Comenius University Bratislava, Faculty of Mathematics, Physics and Informatics, Bratislava, Slovakia}}
\newcommand{\JUNOBT}{\affiliation{Department of Physics, Faculty of Science, Chulalongkorn University, Bangkok, Thailand}}
\newcommand{\JUNOBU}{\affiliation{National Astronomical Research Institute of Thailand, Chiang Mai, Thailand}}
\newcommand{\JUNOBV}{\affiliation{Suranaree University of Technology, Nakhon Ratchasima, Thailand}}
\newcommand{\JUNOBW}{\affiliation{Department of Physics and Astronomy, University of California, Irvine, California, USA}}


\author{A.~Abusleme}\JUNOE
\author{T.~Adam}\JUNOAS
\author{S.~Ahmad}\JUNOBO
\author{R.~Ahmed}\JUNOBO
\author{S.~Aiello}\JUNOBC
\author{F.~P.~An}\JUNOAC
\author{G.~P.~An}\IHEP
\author{Q.~An}\USTC
\author{G.~Andronico}\JUNOBC
\author{N.~Anfimov}\Dubna
\author{V.~Antonelli}\JUNOBF
\author{T.~Antoshkina}\Dubna
\author{B.~Asavapibhop}\JUNOBT
\author{J.~P.~A.~M.~de Andr\'{e}}\JUNOAS
\author{D.~Auguste}\JUNOAQ
\author{A.~Babic}\JUNOBS
\author{W.~Baldini}\JUNOBE
\author{A.~Barresi}\JUNOBG
\author{E.~Baussan}\JUNOAS
\author{M.~Bellato}\JUNOBI
\author{A.~Bergnoli}\JUNOBI
\author{E.~Bernieri}\JUNOBM
\author{T.~Birkenfeld}\JUNOAV
\author{S.~Blin}\JUNOAQ
\author{D.~Blum}\JUNOBB
\author{S.~Blyth}\NTU
\author{A.~Bolshakova}\Dubna
\author{M.~Bongrand}\JUNOAQ
\author{C.~Bordereau}\JUNOAR\NUU
\author{D.~Breton}\JUNOAQ
\author{A.~Brigatti}\JUNOBF
\author{R.~Brugnera}\JUNOBJ
\author{R.~Bruno}\JUNOBC
\author{A.~Budano}\JUNOBM
\author{M.~Buesken}\JUNOAV
\author{M.~Buscemi}\JUNOBC
\author{Jose Busto}\JUNOAT
\author{I.~Butorov}\Dubna
\author{A.~Cabrera}\JUNOAQ
\author{H.~Cai}\JUNOAH
\author{X.~Cai}\IHEP
\author{Y.~K.~Cai}\IHEP
\author{Z.~Y.~Cai}\IHEP
\author{A.~Cammi}\JUNOBH
\author{A.~Campeny}\JUNOE
\author{C.~Y.~Cao}\IHEP
\author{G.~F.~Cao}\IHEP
\author{J.~Cao}\IHEP
\author{R.~Caruso}\JUNOBC
\author{C.~Cerna}\JUNOAR
\author{I.~Chakaberia}\SDU
\author{J.~F.~Chang}\IHEP
\author{Y.~Chang}\NUU
\author{P.~P.~Chen}\JUNOR
\author{P.~A.~Chen}\NTU
\author{S.~Chen}\TSINGHUA
\author{X.~Chen}\JUNOZ
\author{Y.~W.~Chen}\NCTU
\author{Y.~Chen}\NCEPU
\author{Y.~Chen}\ZSU
\author{Z.~Chen}\IHEP
\author{J.~Cheng}\IHEP
\author{Y.~Cheng}\JUNOG
\author{D.~Chiesa}\JUNOBG
\author{P.~Chimenti}\JUNOC
\author{A.~Chukanov}\Dubna
\author{A.~Chuvashova}\Dubna
\author{G.~Claverie}\JUNOAR
\author{C.~Clementi}\JUNOBK
\author{B.~Clerbaux}\JUNOB
\author{S.~Di Lorenzo}\JUNOAQ
\author{D.~Corti}\JUNOBI
\author{S.~Costa}\JUNOBC
\author{F.~D.~Corso}\JUNOBI
\author{O.~Dalager}\UCI
\author{C.~De La Taille}\JUNOAQ
\author{J.~Deng}\JUNOAH
\author{Z.~Deng}\TSINGHUA
\author{Z.~Y.~Deng}\IHEP
\author{W.~Depnering}\JUNOAZ
\author{M.~Diaz}\JUNOE
\author{X.~F.~Ding}\JUNOBF
\author{Y.~Y.~Ding}\IHEP
\author{B.~Dirgantara}\JUNOBV
\author{S.~Dmitrievsky}\Dubna
\author{T.~Dohnal}\Charles
\author{G.~Donchenko}\JUNOBR
\author{J.~M.~Dong}\TSINGHUA
\author{D.~Dornic}\JUNOAT
\author{E.~Doroshkevich}\JUNOBQ
\author{M.~Dracos}\JUNOAS
\author{F.~Druillole}\JUNOAR
\author{S.~X.~Du}\JUNOAK
\author{S.~Dusini}\JUNOBI
\author{M.~Dvorak}\Charles
\author{T.~Enqvist}\JUNOAP
\author{H.~Enzmann}\JUNOAZ
\author{A.~Fabbri}\JUNOBM
\author{L.~Fajt}\JUNOBS
\author{D.~H.~Fan}\JUNOX
\author{L.~Fan}\IHEP
\author{C.~Fang}\JUNOAB
\author{J.~Fang}\IHEP
\author{W.~X.~Fang}\IHEP
\author{M.~Fargetta}\JUNOBC
\author{A.~Fatkina}\Dubna
\author{D.~Fedoseev}\Dubna
\author{V.~Fekete}\JUNOBS
\author{L.~C.~Feng}\NCTU
\author{Q.~C.~Feng}\JUNOU
\author{R.~Ford}\JUNOBF
\author{A.~Formozov}\JUNOBF
\author{A.~Fournier}\JUNOAR
\author{H.~N.~Gan}\JUNOF
\author{F.~Gao}\JUNOAV
\author{A.~Garfagnini}\JUNOBJ
\author{A.~G\"{o}ttel}\JUNOAX\JUNOAV
\author{C.~Genster}\JUNOAX
\author{M.~Giammarchi}\JUNOBF
\author{A.~Giaz}\JUNOBJ
\author{N.~Giudice}\JUNOBC
\author{M.~Gonchar}\Dubna
\author{G.~Gong}\TSINGHUA
\author{H.~Gong}\TSINGHUA
\author{O.~Gorchakov}\Dubna
\author{Y.~Gornushkin}\Dubna
\author{M.~Grassi}\JUNOBJ
\author{C.~Grewing}\JUNOAY
\author{V.~Gromov}\Dubna
\author{M.~Gu}\IHEP
\author{X.~Gu}\JUNOAK
\author{Y.~Gu}\JUNOS
\author{M.~Y.~Guan}\IHEP
\author{N.~Guardone}\JUNOBC
\author{M.~Gul}\JUNOBO
\author{C.~Guo}\IHEP
\author{J.~Y.~Guo}\ZSU
\author{W.~L.~Guo}\IHEP
\author{X.~H.~Guo}\BNU
\author{Y.~H.~Guo}\JUNOAX
\author{P.~Hackspacher}\JUNOAZ
\author{C.~Hagner}\JUNOAW
\author{R.~Han}\JUNOG
\author{Y.~Han}\JUNOAQ
\author{M.~Hassan}\JUNOBO
\author{M.~He}\IHEP
\author{W.~He}\IHEP
\author{T.~Heinz}\JUNOBB
\author{P.~Hellmuth}\JUNOAR
\author{Y.~K.~Heng}\IHEP
\author{R.~Herrera}\JUNOE
\author{D.~J.~Hong}\JUNOAB
\author{S.~J.~Hou}\IHEP
\author{Y.~Hsiung}\NTU
\author{B.~Z.~Hu}\NTU
\author{H.~Hu}\ZSU
\author{J.~R.~Hu}\IHEP
\author{J.~Hu}\IHEP
\author{S.~Y.~Hu}\CIAE
\author{T.~Hu}\IHEP
\author{Z.~J.~Hu}\ZSU
\author{C.~H.~Huang}\ZSU
\author{G.~H.~Huang}\IHEP
\author{H.~X.~Huang}\CIAE
\author{Q.~H.~Huang}\JUNOAS
\author{W.~H.~Huang}\SDU
\author{X.~Huang}\IHEP
\author{X.~T.~Huang}\SDU
\author{Y.~B.~Huang}\JUNOAB
\author{J.~Q.~Hui}\JUNOAD
\author{L.~Huo}\JUNOU
\author{W.~Huo}\USTC
\author{C.~Huss}\JUNOAR
\author{S.~Hussain}\JUNOBO
\author{A.~Insolia}\JUNOBC
\author{A.~Ioannisian}\JUNOA
\author{R.~Isocrate}\JUNOBI
\author{K.~L.~Jen}\NCTU
\author{X.~L.~Ji}\IHEP
\author{X.~Z.~Ji}\ZSU
\author{H.~H.~Jia}\NanKai
\author{J.~J.~Jia}\JUNOAH
\author{S.~Y.~Jian}\CIAE
\author{D.~Jiang}\USTC
\author{X.~S.~Jiang}\IHEP
\author{R.~Y.~Jin}\IHEP
\author{X.~P.~Jing}\IHEP
\author{C.~Jollet}\JUNOAR
\author{J.~Joutsenvaara}\JUNOAP
\author{S.~Jungthawan}\JUNOBV
\author{L.~Kalousis}\JUNOAS
\author{P.~Kampmann}\JUNOAX\JUNOAV
\author{L.~Kang}\JUNOR
\author{M.~Karagounis}\JUNOAY
\author{N.~Kazarian}\JUNOA
\author{A.~Khan}\ZSU
\author{W.~Khan}\JUNOAI
\author{K.~Khosonthongkee}\JUNOBV
\author{P.~Kinz}\NCTU
\author{D.~Korablev}\Dubna
\author{K.~Kouzakov}\JUNOBR
\author{A.~Krasnoperov}\Dubna
\author{Z.~Krumshteyn}\Dubna
\author{A.~Kruth}\JUNOAY
\author{N.~Kutovskiy}\Dubna
\author{P.~Kuusiniemi}\JUNOAP
\author{T.~Lachenmaier}\JUNOBB
\author{C.~Landini}\JUNOBF
\author{S.~Leblanc}\JUNOAR
\author{V.~Lebrin}\JUNOAU
\author{F.~Lefevre}\JUNOAU
\author{R.~Lei}\JUNOR
\author{R.~Leitner}\Charles
\author{J.~Leung}\NCTU
\author{C.~Li}\SDU
\author{D.~Li}\JUNOAK
\author{F.~Li}\IHEP
\author{F.~Li}\TSINGHUA
\author{H.~Li}\ZSU
\author{H.~L.~Li}\IHEP
\author{J.~Li}\ZSU
\author{K.~J.~Li}\ZSU
\author{M.~Z.~Li}\IHEP
\author{M.~Li}\NCEPU
\author{N.~Li}\NUDT
\author{N.~Li}\IHEP
\author{Q.~J.~Li}\NUDT
\author{R.~H.~Li}\IHEP
\author{S.~F.~Li}\JUNOR
\author{S.~J.~Li}\ZSU
\author{T.~Li}\ZSU
\author{T.~Li}\SDU
\author{W.~D.~Li}\IHEP
\author{W.~G.~Li}\IHEP
\author{X.~M.~Li}\CIAE
\author{X.~N.~Li}\IHEP
\author{X.~L.~Li}\CIAE
\author{Y.~Li}\JUNOR
\author{Y.~F.~Li}\IHEP
\author{Z.~Li}\IHEP
\author{Z.~B.~Li}\ZSU
\author{Z.~Y.~Li}\ZSU
\author{H.~Liang}\USTC
\author{H.~Liang}\CIAE
\author{J.~J.~Liang}\JUNOAB
\author{D.~Liebau}\JUNOAY
\author{A.~Limphirat}\JUNOBV
\author{S.~Limpijumnong}\JUNOBV
\author{G.~L.~Lin}\NCTU
\author{S.~X.~Lin}\JUNOR
\author{T.~Lin}\IHEP
\author{J.~J.~Ling}\ZSU
\author{I.~Lippi}\JUNOBI
\author{F.~Liu}\NCEPU
\author{H.~D.~Liu}\JUNOAK
\author{H.~B.~Liu}\JUNOAB
\author{H.~J.~Liu}\JUNOW
\author{H.~T.~Liu}\ZSU
\author{H.~Liu}\ZSU
\author{H.~Liu}\JUNOS
\author{J.~L.~Liu}\JUNOAD\JUNOAE
\author{J.~C.~Liu}\IHEP
\author{M.~Liu}\JUNOW
\author{Q.~Liu}\JUNON
\author{Q.~Liu}\USTC
\author{R.~X.~Liu}\JUNOAX\JUNOAV
\author{S.~Y.~Liu}\IHEP
\author{S.~B.~Liu}\USTC
\author{S.~L.~Liu}\IHEP
\author{X.~W.~Liu}\ZSU
\author{X.~Liu}\JUNOAB
\author{Y.~Liu}\IHEP
\author{Y.~Liu}\IHEP
\author{A.~Lokhov}\JUNOBR
\author{P.~Lombardi}\JUNOBF
\author{C.~Lombardo}\JUNOBD
\author{K.~Loo}\JUNOAZ
\author{C.~Lu}\JUNOAF
\author{H.~Q.~Lu}\IHEP
\author{J.~B.~Lu}\JUNOO
\author{J.~G.~Lu}\IHEP
\author{S.~X.~Lu}\JUNOAK
\author{X.~X.~Lu}\IHEP
\author{B.~Lubsandorzhiev}\JUNOBQ
\author{S.~Lubsandorzhiev}\JUNOBQ
\author{L.~Ludhova}\JUNOAX\JUNOAV
\author{F.~J.~Luo}\IHEP
\author{G.~Luo}\ZSU
\author{P.~W.~Luo}\ZSU
\author{S.~Luo}\JUNOAJ
\author{W.~M.~Luo}\IHEP
\author{V.~Lyashuk}\JUNOBQ
\author{Q.~M.~Ma}\IHEP
\author{S.~Ma}\IHEP
\author{X.~Y.~Ma}\IHEP
\author{X.~B.~Ma}\NCEPU
\author{J.~Maalmi}\JUNOAQ
\author{Y.~Malyshkin}\Dubna
\author{F.~Mantovani}\JUNOBE
\author{F.~Manzali}\JUNOBJ
\author{X.~Mao}\JUNOG
\author{Y.~J.~Mao}\JUNOL
\author{S.~M.~Mari}\JUNOBM
\author{F.~Marini}\JUNOBJ
\author{S.~Marium}\JUNOBO
\author{C.~Martellini}\JUNOBM
\author{G.~Martin-Chassard}\JUNOAQ
\author{A.~Martini}\JUNOBL
\author{D.~Mayilyan}\JUNOA
\author{A.~M\"{u}ller}\JUNOBB
\author{I.~Mednieks}\JUNOBN
\author{Y.~Meng}\JUNOAD
\author{A.~Meregaglia}\JUNOAR
\author{E.~Meroni}\JUNOBF
\author{D.~Meyh\"{o}fer}\JUNOAW
\author{M.~Mezzetto}\JUNOBI
\author{J.~Miller}\JUNOF
\author{L.~Miramonti}\JUNOBF
\author{S.~Monforte}\JUNOBC
\author{P.~Montini}\JUNOBM
\author{M.~Montuschi}\JUNOBE
\author{N.~Morozov}\Dubna
\author{A.~Muhammad}\JUNOBO
\author{P.~Muralidharan}\JUNOAY
\author{M.~Nastasi}\JUNOBG
\author{D.~V.~Naumov}\Dubna
\author{E.~Naumova}\Dubna
\author{I.~Nemchenok}\Dubna
\author{F.~P.~Ning}\IHEP
\author{Z.~Ning}\IHEP
\author{H.~Nunokawa}\JUNOD
\author{L.~Oberauer}\JUNOBA
\author{J.~P.~Ochoa-Ricoux}\UCI\JUNOE
\author{A.~Olshevskiy}\Dubna
\author{D.~Orestano}\JUNOBM
\author{F.~Ortica}\JUNOBK
\author{H.~R.~Pan}\NTU
\author{A.~Paoloni}\JUNOBL
\author{N.~Parkalian}\JUNOAY
\author{S.~Parmeggiano}\JUNOBF
\author{T.~Payupol}\JUNOBT
\author{Y.~Pei}\IHEP
\author{N.~Pelliccia}\JUNOBK
\author{A.~Peng}\JUNOW
\author{H.~Peng}\USTC
\author{F.~Perrot}\JUNOAR
\author{P.~A.~Petitjean}\JUNOB
\author{F.~Petrucci}\JUNOBM
\author{L.~F.~Pi\~{n}eres Rico}\JUNOAS
\author{O.~Pilarczyk}\JUNOAZ
\author{A.~Popov}\JUNOBR
\author{P.~Poussot}\JUNOAS
\author{W.~Pratumwan}\JUNOBV
\author{E.~Previtali}\JUNOBG
\author{F.~Qi}\IHEP
\author{M.~Qi}\NJU
\author{S.~Qian}\IHEP
\author{X.~H.~Qian}\IHEP
\author{H.~Qiao}\JUNOL
\author{Z.~H.~Qin}\IHEP
\author{S.~K.~Qiu}\JUNOW
\author{M.~Rajput}\JUNOBO
\author{G.~Ranucci}\JUNOBF
\author{N.~Raper}\ZSU
\author{A.~Re}\JUNOBF
\author{H.~Rebber}\JUNOAW
\author{A.~Rebii}\JUNOAR
\author{B.~Ren}\JUNOR
\author{J.~Ren}\CIAE
\author{T.~Rezinko}\Dubna
\author{B.~Ricci}\JUNOBE
\author{M.~Robens}\JUNOAY
\author{M.~Roche}\JUNOAR
\author{N.~Rodphai}\JUNOBT
\author{A.~Romani}\JUNOBK
\author{B.~Roskovec}\UCI
\author{C.~Roth}\JUNOAY
\author{X.~Ruan}\JUNOAB
\author{X.~Ruan}\CIAE
\author{S.~Rujirawat}\JUNOBV
\author{A.~Rybnikov}\Dubna
\author{A.~Sadovsky}\Dubna
\author{P.~Saggese}\JUNOBF
\author{G.~Salamanna}\JUNOBM
\author{S.~Sanfilippo}\JUNOBM
\author{A.~Sangka}\JUNOBU
\author{N.~Sanguansak}\JUNOBV
\author{U.~Sawangwit}\JUNOBU
\author{J.~Sawatzki}\JUNOBA
\author{F.~Sawy}\JUNOBJ
\author{M.~Schever}\JUNOAX\JUNOAV
\author{J.~Schuler}\JUNOAS
\author{C.~Schwab}\JUNOAS
\author{K.~Schweizer}\JUNOBA
\author{D.~Selivanov}\Dubna
\author{A.~Selyunin}\Dubna
\author{A.~Serafini}\JUNOBE
\author{G.~Settanta}\JUNOAX
\author{M.~Settimo}\JUNOAU
\author{Z.~Shao}\JUNOAI
\author{V.~Sharov}\Dubna
\author{J.~Shi}\IHEP
\author{V.~Shutov}\Dubna
\author{A.~Sidorenkov}\JUNOBQ
\author{F.~Simkovic}\JUNOBS
\author{C.~Sirignano}\JUNOBJ
\author{J.~Siripak}\JUNOBV
\author{M.~Sisti}\JUNOBG
\author{M.~Slupecki}\JUNOAP
\author{M.~Smirnov}\ZSU
\author{O.~Smirnov}\Dubna
\author{T.~Sogo-Bezerra}\JUNOAU
\author{J.~Songwadhana}\JUNOBV
\author{B.~Soonthornthum}\JUNOBU
\author{A.~Sotnikov}\Dubna
\author{O.~Sramek}\Charles
\author{W.~Sreethawong}\JUNOBV
\author{A.~Stahl}\JUNOAV
\author{L.~Stanco}\JUNOBI
\author{K.~Stankevich}\JUNOBR
\author{D.~Stefanik}\JUNOBS
\author{H.~Steiger}\JUNOBA
\author{J.~Steinmann}\JUNOAV
\author{T.~Sterr}\JUNOBB
\author{M.~R.~Stock}\JUNOBA
\author{V.~Strati}\JUNOBE
\author{A.~Studenikin}\JUNOBR
\author{G.~X.~Sun}\IHEP
\author{S.~F.~Sun}\NCEPU
\author{X.~L.~Sun}\IHEP
\author{Y.~J.~Sun}\USTC
\author{Y.~Z.~Sun}\IHEP
\author{N.~Suwonjandee}\JUNOBT
\author{M.~Szelezniak}\JUNOAS
\author{J.~Tang}\ZSU
\author{Q.~Tang}\ZSU
\author{Q.~Tang}\JUNOW
\author{X.~Tang}\IHEP
\author{A.~Tietzsch}\JUNOBB
\author{I.~Tkachev}\JUNOBQ
\author{T.~Tmej}\Charles
\author{K.~Treskov}\Dubna
\author{A.~Triossi}\JUNOAS
\author{G.~Troni}\JUNOE
\author{W.~Trzaska}\JUNOAP
\author{C.~Tuve}\JUNOBC
\author{N.~Ushakov}\JUNOBQ
\author{S.~van Waasen}\JUNOAY
\author{J.~Vanden Boom}\JUNOAY
\author{G.~Vanroyen}\JUNOAU
\author{N.~Vassilopoulos}\IHEP
\author{V.~Vedin}\JUNOBN
\author{G.~Verde}\JUNOBC
\author{M.~Vialkov}\JUNOBR
\author{B.~Viaud}\JUNOAU
\author{C.~Volpe}\JUNOAQ
\author{V.~Vorobel}\Charles
\author{D.~Voronin}\JUNOBQ
\author{L.~Votano}\JUNOBL
\author{P.~Walker}\JUNOE
\author{C.~Wang}\JUNOR
\author{C.~H.~Wang}\NUU
\author{E.~Wang}\JUNOAK
\author{G.~Wang}\JUNOU
\author{J.~Wang}\USTC
\author{J.~Wang}\ZSU
\author{K.~Y.~Wang}\IHEP
\author{L.~Wang}\IHEP
\author{M.~F.~Wang}\IHEP
\author{M.~Wang}\SDU
\author{M.~Wang}\JUNOW
\author{R.~G.~Wang}\IHEP
\author{S.~G.~Wang}\JUNOL
\author{W.~Wang}\NJU
\author{W.~Wang}\ZSU
\author{W.~S.~Wang}\IHEP
\author{X.~Wang}\NUDT
\author{X.~Y.~Wang}\ZSU
\author{Y.~F.~Wang}\IHEP
\author{Y.~G.~Wang}\JUNOAH
\author{Y.~Wang}\TSINGHUA
\author{Y.~Wang}\JUNOX
\author{Y.~F.~Wang}\IHEP
\author{Y.~Q.~Wang}\TSINGHUA
\author{Y.~Wang}\NJU
\author{Z.~Wang}\TSINGHUA
\author{Z.~Wang}\IHEP
\author{Z.~M.~Wang}\IHEP
\author{Z.~Y.~Wang}\TSINGHUA
\author{M.~Waqas}\JUNOBO
\author{A.~Watcharangkool}\JUNOBU
\author{L.~H.~Wei}\IHEP
\author{W.~Wei}\IHEP
\author{Y.~D.~Wei}\JUNOR
\author{L.~J.~Wen}\IHEP
\author{C.~Wiebusch}\JUNOAV
\author{S.~C.~F.~Wong}\ZSU
\author{B.~Wonsak}\JUNOAW
\author{D.~Wu}\IHEP
\author{F.~L.~Wu}\NJU
\author{Q.~Wu}\SDU
\author{W.~J.~Wu}\JUNOAH
\author{Z.~Wu}\IHEP
\author{M.~Wurm}\JUNOAZ
\author{J.~Wurtz}\JUNOAS
\author{C.~Wysotzki}\JUNOAV
\author{Y.~F.~Xi}\JUNOAF
\author{D.~M.~Xia}\CQU
\author{Y.~G.~Xie}\IHEP
\author{Z.~Q.~Xie}\IHEP
\author{Z.~Z.~Xing}\IHEP
\author{B.~Xu}\TSINGHUA
\author{C.~Xu}\JUNOW
\author{D.~L.~Xu}\JUNOAE\JUNOAD
\author{F.~R.~Xu}\JUNOS
\author{H.~K.~Xu}\IHEP
\author{J.~L.~Xu}\IHEP
\author{J.~Xu}\BNU
\author{M.~H.~Xu}\IHEP
\author{Y.~Xu}\NanKai
\author{Y.~Xu}\JUNOAX\JUNOAV
\author{B.~J.~Yan}\IHEP
\author{T.~Yan}\JUNOBV
\author{W.~Q.~Yan}\IHEP
\author{X.~B.~Yan}\IHEP
\author{Y.~P.~Yan}\JUNOBV
\author{A.~B.~Yang}\IHEP
\author{C.~G.~Yang}\IHEP
\author{H.~Yang}\IHEP
\author{J.~Yang}\JUNOAK
\author{L.~Yang}\JUNOR
\author{X.~Y.~Yang}\IHEP
\author{Y.~.~Yang}\JUNOB
\author{Y.~F.~Yang}\IHEP
\author{H.~F.~Yao}\IHEP
\author{Z.~Yasin}\JUNOBO
\author{J.~X.~Ye}\IHEP
\author{M.~Ye}\IHEP
\author{Z.~P.~Ye}\JUNOAE
\author{U.~Yegin}\JUNOAY
\author{F.~Yermia}\JUNOAU
\author{P.~H.~Yi}\IHEP
\author{X.~W.~Yin}\IHEP
\author{Z.~Y.~You}\ZSU
\author{B.~X.~Yu}\IHEP
\author{C.~Y.~Yu}\JUNOR
\author{C.~X.~Yu}\NanKai
\author{H.~Z.~Yu}\ZSU
\author{M.~Yu}\JUNOAH
\author{X.~H.~Yu}\NanKai
\author{Z.~Y.~Yu}\IHEP
\author{C.~Z.~Yuan}\IHEP
\author{Y.~Yuan}\JUNOL
\author{Z.~X.~Yuan}\TSINGHUA
\author{Z.~Y.~Yuan}\JUNOAH
\author{B.~B.~Yue}\ZSU
\author{N.~Zafar}\JUNOBO
\author{A.~Zambanini}\JUNOAY
\author{S.~Zeng}\IHEP
\author{T.~X.~Zeng}\IHEP
\author{Y.~D.~Zeng}\ZSU
\author{L.~Zhan}\IHEP
\author{F.~Y.~Zhang}\JUNOAD
\author{G.~Q.~Zhang}\IHEP
\author{H.~Q.~Zhang}\IHEP
\author{H.~H.~Zhang}\ZSU
\author{J.~W.~Zhang}\IHEP
\author{J.~Zhang}\IHEP
\author{J.~B.~Zhang}\JUNOU
\author{J.~Zhang}\IHEP
\author{P.~Zhang}\IHEP
\author{Q.~M.~Zhang}\JUNOAI
\author{S.~Zhang}\ZSU
\author{S.~Zhang}\ZSU
\author{T.~Zhang}\JUNOAD
\author{X.~M.~Zhang}\IHEP
\author{X.~T.~Zhang}\IHEP
\author{Y.~Zhang}\IHEP
\author{Y.~H.~Zhang}\IHEP
\author{Y.~Y.~Zhang}\IHEP
\author{Y.~P.~Zhang}\IHEP
\author{Y.~Y.~Zhang}\JUNOAD
\author{Y.~M.~Zhang}\ZSU
\author{Z.~Y.~Zhang}\JUNOAH
\author{Z.~J.~Zhang}\JUNOR
\author{F.~Y.~Zhao}\JUNOZ
\author{J.~Zhao}\IHEP
\author{R.~Zhao}\ZSU
\author{S.~J.~Zhao}\JUNOAK
\author{T.~C.~Zhao}\IHEP
\author{D.~Q.~Zheng}\JUNOS
\author{H.~Zheng}\JUNOR
\author{M.~S.~Zheng}\CIAE
\author{Y.~H.~Zheng}\JUNON
\author{W.~R.~Zhong}\JUNOS
\author{J.~Zhou}\CIAE
\author{L.~Zhou}\IHEP
\author{N.~Zhou}\USTC
\author{S.~Zhou}\IHEP
\author{X.~Zhou}\JUNOAH
\author{J.~Zhu}\ZSU
\author{K.~J.~Zhu}\IHEP
\author{B.~Zhuang}\IHEP
\author{H.~L.~Zhuang}\IHEP
\author{L.~Zong}\TSINGHUA
\author{J.~H.~Zou}\IHEP
\collaboration{The JUNO Collaboration}
\noaffiliation


%%%%%%%%%%%%%%%%%%%%%%%%
%MTAS
%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\PDORNL}{\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, TN, USA}}
\author{B.~C.~Rasco}\PDORNL
%\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, TN, USA}
\collaboration{on behalf of The MTAS Collaboration}
\noaffiliation

%%%%%%%%%%%%%%%%%%%%%%%%
%NEOS
%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\NEOSa}{\affiliation{Department of Physics, Chung-Ang University, Seoul, 06974, Korea}}
\newcommand{\NEOSb}{\affiliation{Center for Underground Physics, Institute for Basic Science (IBS), Daejeon, 34126, Korea}}
\newcommand{\NEOSc}{\affiliation{Neutron Science Division, Korea Atomic Energy Research Institute, Deajeon, 34057, Korea}}
\newcommand{\NEOSd}{\affiliation{Center for Ionizing Radiation, Korea Research Institute of Standards and Science, Daejeon, 34113, Korea}}
\newcommand{\NEOSe}{\affiliation{Department of Accelerator Science, Korea University, Sejong, 30019, Korea}}
\newcommand{\NEOSf}{\affiliation{Department of Physics, Kyungpook National University, Daegu, 41566, Korea}}
\newcommand{\NEOSg}{\affiliation{Department of Physics and Astronomy, Sejong University, Seoul, 05006, Korea}}
\newcommand{\NEOSh}{\affiliation{Department of Physics, SungKyun Kwan University, Suwon, 16419, Korea}}
\newcommand{\NEOSi}{\affiliation{IBS School, University of Science and Technology (UST), Daejeon, 34113, Korea}}
\newcommand{\KNU}{\affiliation{Department of Physics, Kyungpook National University, Daegu 41566, Korea}}
\newcommand{\SKKU}{\affiliation{Department of Physics, Sungkyunkwan University, Suwon 16419, Korea}}

\author{B.~Y.~Han}\NEOSc
\author{E.~J.~Jeon}\NEOSb
\author{Y.~Jeong}\NEOSa
\author{H.~S.~Jo}\KNU
\author{D.~K.~Kim}\KNU
\author{J.~Y.~Kim}\NEOSg
\author{J.~G.~Kim}\SKKU
\author{Y.~D.~Kim}\NEOSb\NEOSg\NEOSi
\author{Y.~J.~Ko}\NEOSb
\author{H.~M.~Lee}\NEOSc
\author{M.~H.~Lee}\NEOSb\NEOSi
\author{J.~Lee}\NEOSb
\author{C.~S.~Moon}\KNU
\author{Y.~M.~Oh}\NEOSb
\author{H.~K.~Park}\NEOSe
\author{K.~S.~Park}\NEOSb
\author{S.~H.~Seo}\NEOSb
\author{K.~Siyeon}\NEOSa
\author{G.~M.~Sun}\NEOSc
\author{Y.~S.~Yoon}\NEOSd
\author{I.~Yu}\SKKU

\collaboration{The NEOS Collaboration}
\noaffiliation



%%%%%%%%%%%%%%%
%%% NuLat
%%%%%%%%%%%%%%
\newcommand{\UH}{\affiliation{Department of Physics \& Astronomy, University of Hawaii, Honolulu, HI, USA}}
%\newcommand{\UH}{\affiliation{University of Hawaii, Manoa, HI, USA}}
\newcommand{\NCCU}{\affiliation{North Carolina Central University, Durham, NC, USA}}
\newcommand{\NIST}{\affiliation{National Institute of Standards and Technology, Gaithersburg, MD, USA}}
\newcommand{\VT}{\affiliation{Virginia Tech, Blacksburg, VA, USA}}
\newcommand{\ORNL}{\affiliation{Oak Ridge National Laboratory, Oak Ridge, TN, USA}}
 \newcommand{\NCSDLLNL}{\affiliation{Lawrence Livermore National Laboratory, Livermore, CA, USA}}
 
\author{M.\,J.\,Borusinski}\UH
\author{R.\,Dorrill}\UH
\author{A.\,Druetzler}\UH
\author{J.\,Learned}\UH
\author{V.\,Li}\NCSDLLNL
\author{D.\,Markoff}\NCCU
\author{J.\,Maricic}\UH
\author{S.\,Matsuno}\UH
\author{H.\,P.\,Mumm}\NIST
\author{K.\,Nishimura}\UH
\author{A.\,Irani}\VT
\author{M.\,Pitt}\VT
\author{C.\,Rasco}\ORNL
\author{B.\,Thibodeau}\VT
\author{G.\,Varner}\UH
\author{B.\,Vogelaar}\VT
\author{T.\,Wright}\VT
\collaboration{The NuLat Collaboration}
\noaffiliation


%%%%%%%%%%%%%%%%%%%%%%%%
%PROSPECT
%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\BU}{\affiliation{Department of Physics, Boston University, Boston, MA, USA}}
%\newcommand{\BNL}{\affiliation{Brookhaven National Laboratory, Upton, NY, USA}}
\newcommand{\Drexel}{\affiliation{Department of Physics, Drexel University, Philadelphia, PA, USA}}
\newcommand{\GIT}{\affiliation{George W.\,Woodruff School of Mechanical Engineering, Georgia Institute of Technology, Atlanta, GA USA}}
%\newcommand{\UH}{\affiliation{Department of Physics \& Astronomy, University of Hawaii, Honolulu, HI, USA}}
%\newcommand{\IIT}{\affiliation{Department of Physics, Illinois Institute of Technology, Chicago, IL, USA}}
%\newcommand{\NCSDLLNL}{\affiliation{Lawrence Livermore National Laboratory, Livermore, CA, USA}}
\newcommand{\LeMoyne}{\affiliation{Department of Physics, Le Moyne College, Syracuse, NY, USA}}
\newcommand{\MIT}{\affiliation{Department of Physiscs, Massachusetts Institute of Technology, Cambridge, MA, USA}}
%\newcommand{\NIST}{\affiliation{National Institute of Standards and Technology, Gaithersburg, MD, USA}}
\newcommand{\HFIRORNL}{\affiliation{High Flux Isotope Reactor, Oak Ridge National Laboratory, Oak Ridge, TN, USA}}
%\newcommand{\PDORNL}{\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, TN, USA}}
% \newcommand{\Temple}{\affiliation{Department of Physics, Temple University, Philadelphia, PA, USA}}
\newcommand{\UT}{\affiliation{Department of Physics and Astronomy, University of Tennessee, Knoxville, TN, USA}}
\newcommand{\Waterloo}{\affiliation{Institute for Quantum Computing and Department of Physics and Astronomy, University of Waterloo, Waterloo, ON, Canada}}
% \newcommand{\UWis}{\affiliation{Department of Physics, University of Wisconsin, Madison, Madison, WI, USA}}
%\newcommand{\Yale}{\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, CT, USA}}

\author{M.\,Andriamirado}\IIT
\author{A.\,B.\,Balantekin}\Wisconsin
\author{H.\,R.\,Band}\Yale
\author{C.\,D.\,Bass}\LeMoyne
\author{D.\,E.\,Bergeron}\NIST
\author{D.\,Berish}\TempleUniversity
\author{N.\,S.\,Bowden}\NCSDLLNL
\author{J.\,P.\,Brodsky}\NCSDLLNL
\author{C.\,D.\,Bryan}\HFIRORNL
\author{R.~Carr}\MIT
\author{T.\,Classen}\NCSDLLNL
\author{A.\,J.\,Conant}\ORNL
\author{G.\,Deichert}\HFIRORNL
\author{M.\,V.\,Diwan}\BNL
\author{M.\,J.\,Dolinski}\Drexel
\author{A.\,Erickson}\GIT
\author{B.\,T.\,Foust}\Yale
\author{J.\,K.\,Gaison}\Yale
\author{A.\,Galindo-Uribarri}\PDORNL\UT
\author{C.\,E.\,Gilbert}\PDORNL\UT
\author{C.\,Grant}\BU
\author{B.\,T.\,Hackett}\PDORNL\UT
\author{S.\,Hans}\BNL
\author{A.\,B.\,Hansell}\TempleUniversity
\author{K.\,M.\,Heeger}\Yale
\author{D.\,E.\,Jaffe}\BNL
\author{X.\,Ji}\BNL
\author{D.\,C.\,Jones}\TempleUniversity
\author{O.\,Kyzylova}\Drexel
\author{C.\,E.\,Lane}\Drexel
\author{T.\,J.\,Langford}\Yale
\author{J.\,LaRosa}\NIST
\author{B.\,R.\,Littlejohn}\IIT
\author{X.\,Lu}\PDORNL\UT
\author{J.\,Maricic}\UH
\author{M.\,P.\,Mendenhall}\NCSDLLNL
\author{A.\,M.\,Meyer}\UH
\author{R.\,Milincic}\UH
\author{I.\,Mitchell}\UH
\author{P.\,E.\,Mueller}\PDORNL
\author{H.\,P.\,Mumm}\NIST
\author{J.\,Napolitano}\TempleUniversity
\author{C.\,Nave}\Drexel
\author{R.\,Neilson}\Drexel
\author{J.\,A.\,Nikkel}\Yale
\author{D.\,Norcini}\Yale
\author{S.\,Nour}\NIST
\author{J.\,L.\,Palomino}\IIT
\author{D.\,A.\,Pushin}\Waterloo
\author{X.\,Qian}\BNL
\author{E.\,Romero-Romero}\PDORNL\UT
\author{R.\,Rosero}\BNL
\author{P.\,T.\,Surukuchi}\Yale
\author{M.\,A.\,Tyra}\NIST
\author{R.\,L.\,Varner}\PDORNL
\author{D.\,Venegas-Vargas}\PDORNL\UT
\author{P.\,B.\,Weatherly}\Drexel
\author{C.\,White}\IIT
\author{J.\,Wilhelmi}\Yale
\author{A.\,Woolverton}\Waterloo
\author{M.\,Yeh}\BNL
\author{A.\,Zhang}\BNL
\author{C.\,Zhang}\BNL
\author{X.\,Zhang}\NCSDLLNL
\collaboration{The PROSPECT Collaboration}
\noaffiliation

%%%%%%%%%%%%%%%%%%%%%%%%
%RENO
%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\CNU}{\affiliation{Institute for Universe and Elementary Particles, Chonnam National University, Gwangju 61186, Korea}}
\newcommand{\DSU}{\affiliation{Institute for High Energy Physics, Dongshin University, Naju 58245, Korea}}
\newcommand{\GIST}{\affiliation{GIST College, Gwangju Institute of Science and Technology, Gwangju 61005, Korea}}
\newcommand{\IBS}{\affiliation{Institute for Basic Science, Daejeon 34047, Korea}}
\newcommand{\KAIST}{\affiliation{Department of Physics, KAIST, Daejeon 34141, Korea}}
% \newcommand{\KNU}{\affiliation{Department of Physics, Kyungpook National University, Daegu 41566, Korea}}
\newcommand{\SNU}{\affiliation{Department of Physics and Astronomy, Seoul National University, Seoul 08826, Korea}}
\newcommand{\SYU}{\affiliation{Department of Fire Safety, Seoyeong University, Gwangju 61268, Korea}}
% \newcommand{\SKKU}{\affiliation{Department of Physics, Sungkyunkwan University, Suwon 16419, Korea}}

%\author{G.~Bak}\CNU
\author{J.~H.~Choi}\DSU
\author{H.~I.~Jang}\SYU
\author{J.~S.~Jang}\GIST
\author{S.~H.~Jeon}\SKKU
\author{K.~K.~Joo}\CNU
\author{K.~Ju}\KAIST
\author{D.~E.~Jung}\SKKU
\author{J.~G.~Kim}\SKKU
\author{J.~H.~Kim}\SKKU
\author{J.~Y.~Kim}\CNU
\author{S.~B.~Kim}\SKKU
\author{S.~Y.~Kim}\SNU
\author{W.~Kim}\KNU
\author{E.~Kwon}\SKKU
\author{D.~H.~Lee}\SKKU
\author{H.~G.~Lee}\SNU
\author{I.~T.~Lim}\CNU
\author{D.~H.~Moon}\CNU
\author{M.~Y.~Pac}\DSU
\author{H.~Seo}\SNU
\author{J.~W.~Seo}\SKKU
\author{C.~D.~Shin}\CNU
\author{B.~S.~Yang}\IBS
\author{J.~Yoo}\IBS\KAIST
\author{S.~G. Yoon}\KAIST
\author{I.~S.~Yeo}\CNU
\author{I.~Yu}\SKKU

\collaboration{The RENO Collaboration}
\noaffiliation

%%%%%%%%%%%%%%%%%%%%%%%%
%Ricochet
%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ARGONNE}{\affiliation{Argonne National Laboratory, USA}}
\newcommand{\CSNSM}{\affiliation{Centre de Sciences Nucléaires et de Sciences de la Matière (CSNSM), France}}
\newcommand{\GRENOBLE}{\affiliation{Institut Neel PI at Neel Institute Grenoble, France}}
\newcommand{\LYON}{\affiliation{Institut de Physique Nucléaire de Lyon (IPNL), France}}
\newcommand{\JINR}{\affiliation{Joint Institute for Nuclear Research (JINR), Russian Federation}}
\newcommand{\LPSC}{\affiliation{Laboratoire de Physique Subatomique et de Cosmologie (LPSC), France}}
\newcommand{\MITR}{\affiliation{Massachusetts Institute of Technology, USA}}
\newcommand{\NORTHWESTERN}{\affiliation{Northwestern University, USA}}
\newcommand{\AMHERST}{\affiliation{University of Massachusetts at Amherst, USA}}
\newcommand{\WISC}{\affiliation{University of Wisconsin, USA}}
\newcommand{\LINCOLN}{\affiliation{Lincoln Laboratories, USA}}

\author{C.~Chang}\ARGONNE

\author{L.~Bergé}\CSNSM
\author{A.~Broniatowski}\CSNSM
\author{L.~Dumoulin}\CSNSM
\author{A.~Giuliani}\CSNSM
\author{M.~Chapellier}\CSNSM
\author{P.~De Marcillac}\CSNSM
\author{S.~Marnieros}\CSNSM
\author{E.~Olivieri}\CSNSM
\author{D.~Poda}\CSNSM

\author{M.~Calvo}\GRENOBLE
\author{J.~Goupy}\GRENOBLE
\author{A.~Monfardini}\GRENOBLE

\author{Q.~Arnaud}\LYON
\author{C.~Augier}\LYON
\author{J.~Billard}\LYON
\author{A.~Cazes}\LYON
\author{J.~Colas}\LYON
\author{J.~Filippini}\LYON
\author{J.~Gascon}\LYON
\author{M.~De Jesus}\LYON
\author{H.~Lattaud}\LYON
\author{A.~Juillard}\LYON
\author{T.~Salagnac}\LYON
\author{T.~Soldner}\LYON

\author{A.~Lubashevskiy}\JINR
\author{E.~Yakushev}\JINR
\author{S.~Rozov}\JINR

\author{J.~Lamblin}\LPSC
\author{B.~Mom}\LPSC
\author{A.~Stutz}\LPSC

\author{J.~A.~Formaggio}\MITR
\author{D.~W.~Mayer}\MITR
\author{J.~Johnston}\MITR
\author{P.~Harrington}\MITR
\author{S.~Heine}\MITR
\author{V.~Sibille}\MITR

\author{R.~Chen}\NORTHWESTERN
\author{E.~Figueroa-Feliciano}\NORTHWESTERN
\author{H.~Ziqing}\NORTHWESTERN

\author{S.~Hertel}\AMHERST
\author{P.~Patel}\AMHERST
\author{D.~Pinckney}\AMHERST
\author{A.~Serafin}\AMHERST
\author{A.~Shilcusky}\AMHERST

\author{N.~Decheine}\WISC
\author{K.~Palladino}\WISC

\author{S.~Weber}\LINCOLN
\author{C.~Hirjibehedin}\LINCOLN
\collaboration{The Ricochet Collaboration}


%%%%%%%%%%%%%%%%%%%%%%%%
%ROADSTR
%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\NCSDLLNL}{\affiliation{
%Nuclear and Chemical Sciences Division, 
%Lawrence Livermore National Laboratory, Livermore, CA, USA}}
\newcommand{\UMich}{\affiliation{University of Michigan,  Ann Arbor,  MI,  USA}}

\author{O.\,A.\,Akindele}\NCSDLLNL
\author{N.\,S.\,Bowden}\NCSDLLNL
\author{L.\,Carman}\NCSDLLNL
\author{T.\,Classen}\NCSDLLNL
\author{S.\,Dazeley}\NCSDLLNL
\author{M.\,Ford}\NCSDLLNL
\author{I.\,Jovanovic}\UMich	\author{V.\,Li}\NCSDLLNL
\author{M.\,P.\,Mendenhall}\NCSDLLNL
\author{F.\,Sutanto}\UMich	
\author{N.\,Zaitseva}\NCSDLLNL
\author{X.\,Zhang}\NCSDLLNL
\collaboration{The ROADSTR Near-Field Working Group}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SoLid
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\newcommand{\aSolid}{\affiliation{Universiteit Antwerpen, Antwerpen, Belgium}}
\newcommand{\bSolid}{\affiliation{University of Bristol, Bristol, UK}}
\newcommand{\cSolid}{affiliation{Vrije Universiteit Brussel, Brussel, Belgium}}
\newcommand{\dSolid}{\affiliation{Normandie Univ, ENSICAEN, UNICAEN, CNRS/IN2P3, LPC Caen, 14000 Caen, France}}
\newcommand{\eSolid}{\affiliation{CERN, 1211 Geneva 23, Switzerland}}
\newcommand{\fSolid}{\affiliation{Universiteit Gent, Gent, Belgium}}
\newcommand{\gSolid}{\affiliation{Imperial College London, Department of Physics, London, United Kingdom}}
\newcommand{\hSolid}{\affiliation{SUBATECH, CNRS/IN2P3, Universit\'e de Nantes, Ecole des Mines de Nantes, Nantes, France}}
\newcommand{\iSolid}{\affiliation{LAL, Univ Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, Orsay, France}}
\newcommand{\jSolid}{\affiliation{University of Oxford, Oxford, UK}}
\newcommand{\kSolid}{\affiliation{SCK-CEN, Belgian Nuclear Research Centre, Mol, Belgium}}
\newcommand{\lSolid}{\affiliation{STFC, Rutherford Appleton Laboratory, Harwell Oxford, and Daresbury Laboratory}} \newcommand{\mSolid}{\affiliation{Institut Universitaire de France, F-75005 Paris, France}}
\newcommand{\nSolid}{\affiliation{Universit\'e Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France}}



%List of authors and their corresponding institute
\author{W.~Beaumont}\aSolid
\author{S.~Binet}\nSolid
\author{I.~Bolognino}\hSolid
\author{M.~Bongrand}\hSolid
\author{J.~Borg}\gSolid
\author{V.~Buridon}\dSolid
\author{H.~Chanal}\nSolid
\author{B.~Coup\'e}\kSolid
\author{P.~Crochet}\nSolid
\author{D.~Cussans}\bSolid
\author{A.~De Roeck}\aSolid\eSolid
\author{D.~Durand}\dSolid
\author{M.~Fallot}\hSolid
\author{D.~Galbinski}\gSolid
\author{S.~Gallego}\dSolid
\author{L.~Giot}\hSolid
\author{B.~Guillon}\dSolid
\author{D.~Henaff}\hSolid
\author{S.~Hayashida}\gSolid
\author{B.~Hosseini}\gSolid
\author{S.~Kalcheva}\kSolid
\author{G.~Lehaut}\dSolid
\author{I.~Michiels}\fSolid
\author{S.~Monteil}\nSolid
\author{D.~Newbold}\bSolid\lSolid
\author{N.~Roy}\iSolid
\author{D.~Ryckbosch}\fSolid
\author{H. Rejeb Sfar}\aSolid
\author{L.~Simard}\iSolid\mSolid
\author{A.~Vacheret}\gSolid
\author{G.~Vandierendonck}\fSolid
\author{S.~Van Dyck}\kSolid
\author{N.~van Remortel}\aSolid
\author{S.~Vercaemer}\aSolid
\author{M.~Verstraeten}\aSolid
\author{B.~Viaud}\hSolid
\author{A.~Weber}\jSolid\lSolid
\author{M.~Yeresko}\nSolid
\author{and F.~Yermia.}\hSolid

\collaboration{The SoLid Collaboration}


%%%%%%%%%%%%%%%%%%%%%%%%
%STEREO
%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\MPIK}{\affiliation{Max-Planck-Institut f\"ur Kernphysik, Saupfercheckweg 1, 69117 Heidelberg, Germany}}

\newcommand{\LAPP}{\affiliation{Univ.~Grenoble Alpes, Universit\'e Savoie Mont Blanc, CNRS/IN2P3, LAPP, 74000 Annecy, France}}

\newcommand{\LPSCG}{\affiliation{Univ.~Grenoble Alpes, CNRS, Grenoble INP, LPSC-IN2P3, 38000 Grenoble, France}}

\newcommand{\CEA}{\affiliation{IRFU, CEA, Universit\'e Paris-Saclay, 91191 Gif-sur-Yvette, France}}

\newcommand{\ILL}{\affiliation{Institut Laue-Langevin, CS 20156, 38042 Grenoble Cedex 9, France}}

\author{A.~Bonhomme}\MPIK\CEA

\author{C.~Buck}\MPIK

\author{P.~del~Amo~Sanchez}\LAPP

\author{I.~El~Atmani}\CEA
%\altaffiliation[Present address: ]{Hassan II University, Faculty of Sciences, A\"in Chock, BP 5366 Maarif, Casablanca 20100, Morocco}

\author{L.~Labit}\LAPP

\author{J.~Lamblin}\LPSCG

\author{A.~Letourneau}\CEA

\author{D.~Lhuillier}\CEA

\author{M.~Licciardi}\LPSCG

\author{M.~Lindner}\MPIK

\author{T.~Materna}\CEA

\author{H.~Pessard}\LAPP

\author{R.~Rogly}\CEA

\author{V.~Savu}\CEA

\author{S.~Schoppmann}\MPIK

\author{T.~Soldner}\ILL

\author{A.~Stutz}\LPSCG

\author{M.~Vialat}\ILL

\collaboration{The \textsc{Stereo} Collaboration}
% \homepage{http://www.stereo-experiment.org}

%%%%%%%%%%%%%%%%%%%%%%%%
%Valencia-Nantes TAGS
%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\IDFC}{\affiliation{Instituto de Física Corpuscular, CSIC-Universitat de Valencia, E-46071 Valencia, Spain}}
% \newcommand{\SUB}{\affiliation{Subatech, CNRS/IN2P3, Univ. of Nantes, IMTA}}
\newcommand{\SUBIMT}{\affiliation{SUBATECH, IMT Atlantique, Université de Nantes, CNRS-IN2P3, F-44307 Nantes, France}}

\author{A.~Algora}\IDFC
\author{A.~Beloeuvre}\hSolid%\SUBIMT
\author{M.~Estienne}\hSolid%\SUBIMT
\author{M.~Fallot}\hSolid%\SUBIMT
\author{L.~Giot}\hSolid%\SUBIMT
\author{R.~Kean}\hSolid%\SUBIMT
\author{A.~Porta}\hSolid%\SUBIMT
\author{J.~L.~Tain}\IDFC
\collaboration{The Valencia-Nantes TAGS Collaboration}
\noaffiliation


%%%%%%%%%%%%%%%%%%%%%%%%
%violeta
%%%%%%%%%%%%%%%%%%%%%%%%
\author{I.~Sidelnik}
\collaboration{on behalf of the vIOLETA Collaboration}
\noaffiliation

%%%%%%%%%%%%%%%%%%%%%%%%
%WATCHMAN
%%%%%%%%%%%%%%%%%%%%%%%%


\author{O. A.  Akindele}\NCSDLLNL
\author{T. Anderson}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{M. Askins}	
\affiliation{University of California at Berkeley, Berkeley,  California 94720,  USA} 
\author{Z. Bagdasarian}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{A. Baldoni}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{A. Barna}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{T. Benson}\Wisconsin	
% \affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA, USA} 
\author{M. Bergevin}	
\NCSDLLNL
\author{A. Bernstein}	
\NCSDLLNL
\author{B. Birrittella}	\Wisconsin
% \affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{S. Bogetic}	
\NCSDLLNL
\author{J. Boissevain}	
\affiliation{University of Pennsylvania,  Philadelphia,  Pennsylvania 19104,  USA} 
\author{J. Borusinki}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{S. Boyd}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{T. Brooks}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{M. (Mat) Budsworth}	
\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{J. Burns}	
\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{M. Calle}	
\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{C. Camilo}	
\BNL
\author{A. Carroll}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{J. Coleman}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{R. Collins}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{C. Connor}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{D. Cowen}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{B. Crow}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{J. Curry}	
\NCSDLLNL
\author{F. Dalnoki-Veress}	
\affiliation{Middlebury Institute of International Studies at Monterey, Monterey, California 93940, USA}
\affiliation{James Martin Center for Nonproliferation Studies, Monterey, California 93940, USA}
\author{D. Danielson}	
\affiliation{University of Chicago, Chicago, IL 60637, USA} 
\author{S. Dazeley}	
\NCSDLLNL
\author{M. Diwan}	
\BNL
\author{S. Dixon}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{L. Drakopoulou}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{A. Druetzler}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{J. Duron}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{S. Dye}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{S. Fargher}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{A. Fienberg}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{V. Fischer}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{R. Foster}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{K. (Kat) Frankiewicz}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{T. Gamble}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{D. Gooding}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{S. Gokhale}	
\BNL
\author{C. Grant}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{R. Gregorio}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{J. Gribble}	
\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{J. Griskevich}\UCI	
%\affiliation{University of California at Irvine,  Irvine,  California 92697,  USA} 
\author{D. Hadley}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{J. He}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{K. Healey}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{J. Hecla}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{G. Holt}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{C. Jabbari}	
\affiliation{Middlebury Institute of International Studies at Monterey} 
\affiliation{James Martin Center for Nonproliferation Studies} 
\author{K. Jewkes}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{I. Jovanovic}	
\UMich 
\author{R. Kaiser}	
\affiliation{University of Glasgow, Glasgow, G12 8QQ, Scotland,} 
\author{M. Keenan}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{P. Keener}	
\affiliation{University of Pennsylvania,  Philadelphia,  Pennsylvania 19104,  USA} 
\author{E. (Liz) Kneale}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{V. Kudryavtsev}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{P. Kunkle}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{J. Learned}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{V. Li}	
\NCSDLLNL
\author{P. Litchfield}	
\affiliation{University of Glasgow, Glasgow, G12 8QQ, Scotland,} 
\author{X. Ran Liu}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{G. Lynch}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{M. Malek}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{J. Maricic}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{P. Marr-Laundrie}\Wisconsin
% \affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{B. Masic}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{C. Mauger}	
\affiliation{University of Pennsylvania,  Philadelphia,  Pennsylvania 19104,  USA} 
\author{N. McCauley}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{C. Metelko}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{R. Mills}	
\affiliation{National Nuclear Laboratory (affiliated with University  of  Liverpool,  Liverpool  L69  3BX,  UK)} 
\author{A. Mitra}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{F. Muheim}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{A. Mullen}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{A. Murphy}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{M. Needham}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{E. Neights}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{K. Nishimura}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{K. Ogren}	
\UMich 
\author{G. Orebi Gann}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{L. Oxborough}\Wisconsin	
% \affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{S. Paling}	
\affiliation{Boulby Underground Laboratory, Loftus, Saltburn-by-the-Sea, Cleveland TS13 4UZ, UK} 
\author{A. Papatyi}	
\affiliation{Pacific Northwest National Laboratory, Richland, WA 99352, USA } 
\author{B. Paulos}\Wisconsin	
% \affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{T. Pershing}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{L. Pickard}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{S. Quillin}	
\affiliation{Atomic Weapons Establishment,  Aldermaston,  Reading RG7 4PR, UK} 
\author{R. Resoro}	
\BNL
\author{B. Richards}	
\affiliation{University of Warwick, Coventry, CV4 7AL, UK} 
\author{L. Sabarots}\Wisconsin	
% \affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{A. Scarff}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{Yan-Jie Schnellbach}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{P. Scovell}	
\affiliation{Boulby Underground Laboratory, Loftus, Saltburn-by-the-Sea, Cleveland TS13 4UZ, UK} 
\author{B. Seitz}	
\affiliation{University of Glasgow, Glasgow, G12 8QQ, Scotland,} 
\author{O. Shea}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{V. Shebalin}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{G. Smith}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{M. Smy}	\UCI
%\affiliation{University of California at Irvine,  Irvine,  California 92697,  USA} 
\author{H. Song}	
\affiliation{Boston  University,  Boston,  Massachusetts  02215,  USA} 
\author{N. Spooner}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{C. Stanton}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{O. Stone}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{F. Sutanto}	
\UMich 
\author{R. Svoboda}	
\affiliation{Department of Physics, University of California at Davis, Davis, California 95616, USA} 
\author{S. Szoldos}	
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA} 
\author{L. Thompson}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{F. Thomson}	
\affiliation{University of Glasgow, Glasgow, G12 8QQ, Scotland,} 
\author{C. Toth}	
\affiliation{Boulby Underground Laboratory, Loftus, Saltburn-by-the-Sea, Cleveland TS13 4UZ, UK} 
\author{M. Vagins}\UCI
%\affiliation{University of California at Irvine,  Irvine,  California 92697,  USA} 
\author{R. (Rick) Van Berg}	
\affiliation{University of Pennsylvania,  Philadelphia,  Pennsylvania 19104,  USA} 
\author{G. Varner}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{S. Ventura}	
\affiliation{University of Hawai‘i at M ̄anoa,  Honolulu,  Hawai‘i 96822, USA} 
\author{B. Walsh}	
\BNL
\author{J. Webster}	
\affiliation{The  University  of Edinburgh,  Edinburgh  EH8  9YL, UK} 
\author{M. Weiss}	
\affiliation{Department of Physics, Pennsylvania State University, University Park, Pennsylvania 16802, USA} 
\author{D. Westphal}\NCSDLLNL
\author{M. Wetstein}\IowaState	
%\affiliation{Iowa  State  University,  Ames,  Iowa  50011,  USA} 
\author{T. Wilson}	
\affiliation{University  of  Liverpool,  Liverpool  L69  3BX,  UK} 
\author{S. Wilson}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{S. Wolcott}\Wisconsin	
% \affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA} 
\author{M. Wright}	
\affiliation{The  University  of  Sheffield,  Sheffield  S10  2TN,  UK} 
\author{M. Yeh}	
\BNL
\collaboration{The WATCHMAN collaboration}

%%%%%%%%%%%%%%%%%%%%%%%%
%Uncollab
%%%%%%%%%%%%%%%%%%%%%%%%

\author{J.~M.~Berryman}
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA}\affiliation{University of Kentucky, Lexington, KY}

\author{J.~I.~Collar}
\affiliation{University of Chicago, Chicago, IL 60637, USA} 

\author{A.~Erlandson}\affiliation{Canadian Nuclear Laboratories Ltd., Chalk River, ON, Canada}

\author{S. Gariazzo}\affiliation{Instituto de F{\'\i}sica Corpuscular  (CSIC-Universitat de Val{\`e}ncia),Parc Cient{\'\i}fic UV, C/ Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, E-46980 Paterna (Valencia), Spain}

\author{M.V. Garzelli}\affiliation{University of Hamburg, II Institute for Theoretical Physics}

\author{C.~Giunti}\affiliation{Istituto Nazionale di Fisica Nucleare (INFN), Sezione di Torino, Via P. Giuria 1, I--10125 Torino, Italy}

\author{B.~L.~Goldblum}
\affiliation{University of California at Berkeley, Berkeley, California 94720, USA}

\author{A.~Hayes}\affiliation{Los Alamos National Laboratory, Los Alamos, NM}

\author{S.~Hedges}\Duke %\affiliation{Duke University}

%\author{Y.~F.~Li}\IHEP already in Daya Bay

\author{C.~Mariani}\VirginiaTech

\author{D.~Minic}\VirginiaTech

\author{L.Miramonti}\affiliation{Dipartimento di Fisica, Universita` degli Studi and INFN, 20133 Milano, Italy}

\author{X.~Mougeot}\affiliation{CEA, LIST, Laboratoire National Henri Becquerel, CEA-Saclay 91191 Gif-sur-Yvette Cedex, France}

\author{D.~Naim}\affiliation{University of California, Davis, Davis CA}

\author{J.~Newby}\ORNL
%\affiliation{Oak Ridge National Laboratory, Oak Ridge, TN, USA}

\author{K.~Ni}\affiliation{University of California, San Diego, San Diego, CA}

\author{T.~O'Donnell}\VirginiaTech

\author{S.~Ozturk}\affiliation{Gaziosmanpasa University, Tokat, Turkey}

\author{L.~Périssé}\affiliation{Commissariat à l'Energie Atomique et aux Energies alternatives (CEA)}

\author{R.~Pestes}\VirginiaTech\BNL

\author{A.~A.~Sonzogni}
\affiliation{National Nuclear Data Center, Brookhaven National Laboratory, Upton, NY, USA}


\author{Z.~Tabrizi}\VirginiaTech

\author{M.~Vivier}\CEA
%\affiliation{IRFU, CEA, Université Paris-Saclay, F-91191 Gif-sur-Yvette, France}

\author{K.~Walkup}\VirginiaTech

==> placeholder-Introduction.tex <==
\begin{itemize}
    \item I love lists!
\end{itemize}

\begin{eqnarray}
\label{eq:PMNSMatrix}
U_{PMNS} = \begin{pmatrix} U_{e1} & U_{e2} & U_{e3} & U_{e4} \\ U_{\mu1} & U_{\mu2} & U_{\mu3} & U_{\mu4} \\ U_{\tau1} & U_{\tau2} & U_{\tau3} & U_{\tau4} \\ U_{s1} & U_{s2} & U_{s3} & U_{s4} \\ \end{pmatrix},
\end{eqnarray}
\vspace{1mm} 

\begin{equation}
P_{\nuebar \rightarrow \nuebar} \approx 1 - \sin^22\theta_{14} \sin^2 \frac{\Delta m^2_{41} L}{4E},   
\label{eq:survprob}
\end{equation}

\begin{figure}[hptb!]
\centering
%\includegraphics[trim = 0.0cm 0.0cm 0.0cm 0.0cm, clip=true, width=0.7\textwidth]{figures/Intro_Raa.png}
\includegraphics[trim = 0.0cm 0.0cm 0.0cm 0.0cm, clip=true, width=0.25\textwidth]{figures/blah.pdf}
\caption{I love figures!.  
}
\label{fig:raa}
\end{figure}

I love Figure~\ref{fig:raa}!  

\begin{table*}[thbp!]
\centering
%\vspace{-4mm}
\begin{tabular}{c||c|c|c}
\hline
Experiment & Reactor Type & Scintillator Technology & Search Strategy \\ \hline \hline 
Bugey-3~\cite{Declais:1994su} & Power LEU & Segmented $^6$Li PSD Liquid & Multi-Site \\ \hline 
NEOS~\cite{bib:neos}  & Power LEU & Single-Volume Gd PSD Liquid & Single-Site \\ \hline
DANSS~\cite{danss_osc}  & Power LEU & Segmented Plastic & Multi-Site \\ \hline
STEREO~\cite{stereo_2018}  & Compact HEU & Segmented Gd PSD Liquid & Multi-Zone \\ \hline
PROSPECT~\cite{prospect_osc}  & Compact HEU & Segmented $^6$Li PSD Liquid & Multi-Zone \\ \hline
Neutrino-4~\cite{bib:neutrino4_osc}  & Compact HEU & Segmented Gd Liquid & Multi-Site/Zone \\ \hline

\end{tabular}
\caption{Comparison of experimental parameters of performed reactor-based sterile neutrino search experiments. `Multi-site' means deployment of a detector in multiple locations relative to the reactor. Experiments are listed in rough order of increasing first oscillation publication date.  See text for further details.  
}
\label{tab:current_osc}
\end{table*}
%\end{wraptable}


